Partition Functions, Localization, and the Chiral de Rham complex

We propose a localization formula for the chiral de Rham complex generalizing the well-known localization procedure in topological theories. Our formula takes into account the contribution due to the massive modes. The key to achieve this is to view the non-linear beta-gamma system as a gauge theory. For abelian gauge groups we are in the realm of toric geometry. Including the b-c system, the formula reproduces the known results for the elliptic genus of toric varieties. We compute the partition function of several models.

==> Definitions.tex <==
%PACKAGES

% DRAFT MODE
%\usepackage{showkeys}
%\usepackage{showlabels}
%\usepackage{drafthead}
%\usepackage{draftstamp}
% AMS-Latex packages
\usepackage{latexsym}
\usepackage{amsmath,amssymb,amsxtra,amscd,amsthm}
\usepackage[mathscr]{eucal}
% Package for diagrams
\usepackage[all]{xy}
% Package for indexing
\usepackage{makeidx}
\makeindex
%Package for Young tableaux
%\usepackage[vcentermath]{youngtab}
%Package for Feynman slash
%\usepackage{slashed}
%Package for encapsulated postscript figures
%\usepackage{epsfig}
%Package for Latex2HTML
%\usepackage{html}
%Package for placement of the tables
%\usepackage{flafter}
%\usepackage{datetime}
% Package for synchronization of xemacs and pdf output
%\usepackage{pdfsync}
% Package for thumbnails in pdf documents
%\usepackage{thumbpdf}
% Package for hyperlinks in PDF/PS documents
\usepackage{color}
\usepackage{xr-hyper}
\ifx\pdfoutput\undefined
\usepackage
[dvips,
% pagebackref,
 verbose=false,
 bookmarks=true,
 colorlinks=true,
 linkcolor=webred,
 filecolor=webbrown,
 citecolor=webgreen,
 pagecolor=webblue,
 urlcolor=webblue,
 pdftitle={},
 pdfauthor={Emanuel Scheidegger},
 pdfsubject={},
 pdfkeywords={},
 bookmarksopen=false,
 pdfpagemode=None,
 pdfview=FitH,
 pdfstartview=FitH,
 extension=pdf]{hyperref}
\else
\usepackage
[pdftex,
% pagebackref,
 verbose=false,
 bookmarks=true,
 colorlinks=true,
 linkcolor=webred,
 filecolor=webbrown,
 citecolor=webgreen,
 pagecolor=webblue,
 urlcolor=webblue,
 pdftitle={},
 pdfauthor={Emanuel Scheidegger},
 pdfsubject={},
 pdfkeywords={},
 bookmarksopen=false,
 pdfpagemode=None,
 pdfview=FitH,
 pdfstartview=FitH,
 extension=pdf]{hyperref}
 \pdfcompresslevel=9
 \pdfpagewidth=11truein
 \pdfpageheight=8.5truein
\fi
\definecolor{webred}{rgb}{.8,0,0}
\definecolor{webbrown}{rgb}{.6,0,0}
\definecolor{webgreen}{rgb}{0,0.5,0}
\definecolor{webdkgreen}{rgb}{0,0.3,0}
\definecolor{webblue}{rgb}{0,0,0.5}


%FONTS


% Ralf Smith's Formal Script (rsfs) Font
\DeclareFontFamily{U}{rsfs}{\skewchar\font127 }
\DeclareFontShape{U}{rsfs}{m}{n}{
   <5> rsfs5
   <6> rsfs6
   <7> rsfs7
   <8> rsfs8
   <9> rsfs9
   <10> rsfs10
   <10.95> rsfs11
   <12> rsfs12
   <14.4> rsfs14
   <17.28> rsfs17
   <20.74> rsfs20
   <24.88> rsfs25
   <29.86-> rsfs30}{}
\DeclareMathAlphabet\scr{U}{rsfs}{m}{n}
% Abbreviations for all math fonts (mathcal, mathscr, scr, mathbb, mathfrak)
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}
\def\sA{\mathscr{A}}
\def\sB{\mathscr{B}}
\def\sC{\mathscr{C}}
\def\sD{\mathscr{D}}
\def\sE{\mathscr{E}}
\def\sF{\mathscr{F}}
\def\sG{\mathscr{G}}
\def\sH{\mathscr{H}}
\def\sI{\mathscr{I}}
\def\sJ{\mathscr{J}}
\def\sK{\mathscr{K}}
\def\sL{\mathscr{L}}
\def\sM{\mathscr{M}}
\def\sN{\mathscr{N}}
\def\sO{\mathscr{O}}
\def\sP{\mathscr{P}}
\def\sQ{\mathscr{Q}}
\def\sR{\mathscr{R}}
\def\sS{\mathscr{S}}
\def\sT{\mathscr{T}}
\def\sU{\mathscr{U}}
\def\sV{\mathscr{V}}
\def\sW{\mathscr{W}}
\def\sX{\mathscr{X}}
\def\sY{\mathscr{Y}}
\def\sZ{\mathscr{Z}}
\def\rA{\scr{A}}
\def\rB{\scr{B}}
\def\rC{\scr{C}}
\def\rD{\scr{D}}
\def\rE{\scr{E}}
\def\rF{\scr{F}}
\def\rG{\scr{G}}
\def\rH{\scr{H}}
\def\rI{\scr{I}}
\def\rJ{\scr{J}}
\def\rK{\scr{K}}
\def\rL{\scr{L}}
\def\rM{\scr{M}}
\def\rN{\scr{N}}
\def\rO{\scr{O}}
\def\rP{\scr{P}}
\def\rQ{\scr{Q}}
\def\rR{\scr{R}}
\def\rS{\scr{S}}
\def\rT{\scr{T}}
\def\rU{\scr{U}}
\def\rV{\scr{V}}
\def\rW{\scr{W}}
\def\rX{\scr{X}}
\def\rY{\scr{Y}}
\def\rZ{\scr{Z}}
\def\fA{\mathfrak{A}}
\def\fB{\mathfrak{B}}
\def\fC{\mathfrak{C}}
\def\fD{\mathfrak{D}}
\def\fE{\mathfrak{E}}
\def\fF{\mathfrak{F}}
\def\fG{\mathfrak{G}}
\def\fH{\mathfrak{H}}
\def\fI{\mathfrak{I}}
\def\fJ{\mathfrak{J}}
\def\fK{\mathfrak{K}}
\def\fL{\mathfrak{L}}
\def\fM{\mathfrak{M}}
\def\fN{\mathfrak{N}}
\def\fO{\mathfrak{O}}
\def\fP{\mathfrak{P}}
\def\fQ{\mathfrak{Q}}
\def\fR{\mathfrak{R}}
\def\fS{\mathfrak{S}}
\def\fT{\mathfrak{T}}
\def\fU{\mathfrak{U}}
\def\fV{\mathfrak{V}}
\def\fW{\mathfrak{W}}
\def\fX{\mathfrak{X}}
\def\fY{\mathfrak{Y}}
\def\fZ{\mathfrak{Z}}
\def\fa{\mathfrak{a}}
\def\fb{\mathfrak{b}}
\def\fc{\mathfrak{c}}
\def\fd{\mathfrak{d}}
\def\fe{\mathfrak{e}}
\def\ff{\mathfrak{f}}
\def\fg{\mathfrak{g}}
\def\fh{\mathfrak{h}}
\def\fii{\mathfrak{i}}
\def\fj{\mathfrak{j}}
\def\fk{\mathfrak{k}}
\def\fl{\mathfrak{l}}
\def\fm{\mathfrak{m}}
\def\fn{\mathfrak{n}}
\def\fo{\mathfrak{o}}
\def\fp{\mathfrak{p}}
\def\fq{\mathfrak{q}}
\def\fr{\mathfrak{r}}
\def\fs{\mathfrak{s}}
\def\ft{\mathfrak{t}}
\def\fu{\mathfrak{u}}
\def\fv{\mathfrak{v}}
\def\fw{\mathfrak{w}}
\def\fx{\mathfrak{x}}
\def\fy{\mathfrak{y}}
\def\fz{\mathfrak{z}}
\def\mA{\mathbb{A}}
\def\mB{\mathbb{B}}
\def\mC{\mathbb{C}}
\def\mD{\mathbb{D}}
\def\mE{\mathbb{E}}
\def\mF{\mathbb{F}}
\def\mG{\mathbb{G}}
\def\mH{\mathbb{H}}
\def\mI{\mathbb{I}}
\def\mJ{\mathbb{J}}
\def\mK{\mathbb{K}}
\def\mL{\mathbb{L}}
\def\mM{\mathbb{M}}
\def\mN{\mathbb{N}}
\def\mO{\mathbb{O}}
\def\mP{\mathbb{P}}
\def\mQ{\mathbb{Q}}
\def\mR{\mathbb{R}}
\def\mS{\mathbb{S}}
\def\mT{\mathbb{T}}
\def\mU{\mathbb{U}}
\def\mV{\mathbb{V}}
\def\mW{\mathbb{W}}
\def\mX{\mathbb{X}}
\def\mY{\mathbb{Y}}
\def\mZ{\mathbb{Z}}
\def\tA{\mathrm{A}}
\def\tB{\mathrm{B}}
\def\tC{\mathrm{C}}
\def\tD{\mathrm{D}}
\def\tE{\mathrm{E}}
\def\tF{\mathrm{F}}
\def\tG{\mathrm{G}}
\def\tH{\mathrm{H}}
\def\tI{\mathrm{I}}
\def\tJ{\mathrm{J}}
\def\tK{\mathrm{K}}
\def\tL{\mathrm{L}}
\def\tM{\mathrm{M}}
\def\tN{\mathrm{N}}
\def\tO{\mathrm{O}}
\def\tP{\mathrm{P}}
\def\tQ{\mathrm{Q}}
\def\tR{\mathrm{R}}
\def\tS{\mathrm{S}}
\def\tT{\mathrm{T}}
\def\tU{\mathrm{U}}
\def\tV{\mathrm{V}}
\def\tW{\mathrm{W}}
\def\tX{\mathrm{X}}
\def\tY{\mathrm{Y}}
\def\tZ{\mathrm{Z}}
\def\ta{\mathrm{a}}
\def\tb{\mathrm{b}}
\def\tc{\mathrm{c}}
\def\td{\mathrm{d}}
\def\te{\mathrm{e}}
\def\tf{\mathrm{f}}
\def\tg{\mathrm{g}}
\def\th{\mathrm{h}}
\def\ti{\mathrm{i}}
\def\tj{\mathrm{j}}
\def\tk{\mathrm{k}}
\def\tl{\mathrm{l}}
\def\tm{\mathrm{m}}
\def\tn{\mathrm{n}}
\def\too{\mathrm{o}}
\def\tp{\mathrm{p}}
\def\tq{\mathrm{q}}
\def\trr{\mathrm{r}}
\def\ts{\mathrm{s}}
\def\ttt{\mathrm{t}}
\def\tu{\mathrm{u}}
\def\tv{\mathrm{v}}
\def\tw{\mathrm{w}}
\def\tx{\mathrm{x}}
\def\ty{\mathrm{y}}
\def\tz{\mathrm{z}}

% Font for title page

\newfont{\HUGE}{cmssbx10 scaled 4000}


%MATH SYMBOLS


%Math operator symbols
\DeclareMathOperator{\chern}{ch}
\DeclareMathOperator{\ch}{c}
\DeclareMathOperator{\todd}{td}
\DeclareMathOperator{\p}{p}
\DeclareMathOperator{\sw}{w}
\DeclareMathOperator{\Ar}{\widehat{A}}
\DeclareMathOperator{\rank}{rk}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Det}{Det}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\ext}{ext}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator*{\Res}{Res}
\DeclareMathOperator{\End}{\sE\mathnormal{nd}}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Proj}{Proj}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\ind}{ind}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Supp}{Supp}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\gr}{gr}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\Pexp}{Pexp}
\renewcommand{\Im}{\mathop{\mathrm{Im}}}
\renewcommand{\Re}{\mathop{\mathrm{Re}}}
\renewcommand{\mod}{\mathop{\mathrm{mod}}}
% Blackboard one for unit matrices
\def\bb1{\textup{\small{1}} \kern-3.8pt \textup{1}}
%upright d for differential symbols
\newcommand{\diff}[2]{\textrm{d}^{#1}{#2}}
%exponential function
\newcommand{\e}[1]{\mathrm{e}^{#1}}
% Bra and ket for quantum mechanics
\newcommand{\bra}[1]{\langle #1 |}
\newcommand{\ket}[1]{| #1 \rangle}
\newcommand{\Bra}[1]{\left\langle #1 \right|}
\newcommand{\Ket}[1]{\left| #1 \right\rangle}
\newcommand{\braket}[2]{\langle #1 | #2 \rangle}
\newcommand{\BraKet}[2]{\left\langle #1 \right.\left| #2 \right\rangle}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\lcm}[1]{\textrm{lcm} (#1)}
\def\even{\textrm{even}}
\def\odd{\textrm{odd}}
\def\ev{\mathrm{ev}}
\def\od{\mathrm{od}}
\def\id{\textrm{id}}
\def\eff{\mathrm{eff}}
\def\Coh{\textrm{Coh }}
\def\diag{\textrm{diag}}
\def\Vol{\mathrm{Vol}}
\def\const{\textrm{const }}
\def\ob{\mathrm{ob}}
\def\conv{\mathrm{conv}}
\def\Tot{\mathrm{Tot}}
% Ket for B-type boundary states
\newcommand{\BS}[1]{|\; #1 \;\rangle\!\rangle_B}
% Vectors of different length e.g. for Mori generators
\newcommand{\ve}[7]{(\begin{array}{@{}r@{,}r@{,}r@{,}r@{,}r@{,}r@{,}r@{}}#1&#2&#3&#4&#5&#6&#7 \end{array})}
% Placeholder for a minus sign in lists of vectors
\def\phm{\phantom{-}}
% \nu for extended lattice vector
\def\Bnu{\Bar{\nu}}
% (Extended) Lattice vector of the dual polyhedron of a CY
\newcommand{\dv}[5]{\nu^*_{#1}=(\begin{array}{@{}r@{,}r@{,}r@{,}r@{}}#2&#3&#4&#5 \end{array})}
\newcommand{\dev}[5]{\Bnu^*_{#1}=(\begin{array}{@{}r@{,}r@{,}r@{,}r@{,}r@{}r}#2&#3&#4&#5&\phm1 \end{array})}
% Partial derivative
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
% del and del-bar, CAUTION don't know original meaning of \d
\renewcommand{\d}{\partial}
\newcommand{\dbar}{\bar{\partial}}
% barred i and j and psi
\newcommand{\ibar}{\bar{\imath}}
\newcommand{\jbar}{\bar{\jmath}}
\newcommand{\psibar}{\overline{\psi}}
\newcommand{\phibar}{\overline{\phi}}
\newcommand{\zbar}{\bar{z}}
\newcommand{\Omegabar}{\overline{\Omega}}
\newcommand{\Dbar}{\overline{D}}
\newcommand{\cDbar}{\overline{\cD}}
% Symbol for vector with infinite number of nonnegative integer entries
\def\vk{\vec{k}}
% Short exact sequence
\newcommand{\shortexactseq}[5]{0 \longrightarrow #1 \stackrel{#2}{\longrightarrow} #3 \stackrel{#4}{\longrightarrow} #5 \longrightarrow 0}
% Topological string notation
\newcommand{\F}[1]{\cF^{(#1)}}
\newcommand{\n}[2]{n^{(#1)}_{#2}}
\newcommand{\Li}[1]{\mathrm{Li}_{#1}}
% Notation for toric varieties
\newcommand{\toric}[1]{\mP{\left(\footnotesize\begin{matrix} #1 \end{matrix}\right)}}
\newcommand{\hyp}[1]{\left[\footnotesize\begin{matrix} #1 \end{matrix} \right] }
\newcommand{\neftwo}[2]{\mP{\left(\footnotesize\begin{matrix} #1 \end{matrix} \;\vrule\;\footnotesize\begin{matrix} #2 \end{matrix}\right)}}
\newcommand{\CICYtwo}[2]{\left[\footnotesize\begin{matrix} #1 \end{matrix} \;\vrule\; \footnotesize\begin{matrix} #2 \end{matrix} \right] }
\newcommand{\nefthree}[3]{\mP{\left(\footnotesize\begin{matrix} #1 \end{matrix} \;\vrule\;\footnotesize\begin{matrix} #2 \end{matrix} \;\vrule\;\footnotesize\begin{matrix} #3 \end{matrix}\right)}}
\newcommand{\CICYthree}[3]{\left[\footnotesize\begin{matrix} #1 \end{matrix} \;\vrule\; \footnotesize\begin{matrix} #2 \end{matrix} \;\vrule\; \footnotesize\begin{matrix} #2 \end{matrix} \right] }
% Notation for modular forms
\def\SL2Z{\tS\tL(2,\mZ)}
\def\abcd{\left(\begin{matrix} a & b\\c & d\end{matrix}\right)}
% Text abbreviations
\def\CY{Calabi--Yau }
\def\SCFT{superconformal field theory}
\def\SCA{superconformal algebra}
\def\CFT{conformal field theory}
\def\LG{Landau--Ginzburg}
\def\nlsm{non-linear $\sigma$-model}
\def\glsm{gauged linear $\sigma$-model}
\def\BCFT{boundary conformal field theory}
\def\SYM{super Yang-Mills theory}
\def\CS{Chern--Simons }
\def\PF{Picard--Fuchs }
\renewcommand{\over}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}

%OTHER USEFUL DEFINITIONS

% Equation numbering
\numberwithin{equation}{section}

% Bibliography
\renewcommand\refname{Bibliography}
\providecommand{\href}[2]{#2}

\renewcommand{\labelenumi}{(\alph{enumi})}
\newcommand{\rb}[1]{\raisebox{1.5ex}[-1.5ex]{\textrm{$#1$}}}

% LAYOUT

% normal for articles
%\setlength{\parindent}{0mm}
%\setlength{\textwidth}{15cm}
%\setlength{\oddsidemargin}{6mm}
%\renewcommand{\baselinestretch}{1.2}

% extra wide & long
\setlength{\parindent}{0mm}
\setlength{\textwidth}{180mm}
\setlength{\oddsidemargin}{-10mm}
\setlength{\textheight}{24cm}
\setlength{\topmargin}{-1cm}
\renewcommand{\baselinestretch}{1.2}
\parskip 1ex



% Mathematical Styles
\newtheoremstyle{plain} % name
  {5pt}%      Space above
  {10pt}%      Space below
  {\rmfamily} %         Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\scshape} % Thm head font
  {}%        Punctuation after thm head
  {\newline} %     Space after thm head: " " = normal interword space;
        %       \newline = linebreak
  {}%         Thm head spec (can be left empty, meaning `normal')
\swapnumbers
\theoremstyle{break}
\newtheorem{defin}{Definition}%[subsubsection]
\newtheorem{rem}[defin]{Remark}
\newtheorem{expl}[defin]{Example}
\newtheorem{expls}[defin]{Examples}
\newtheorem{prop}[defin]{Proposition}
\newtheorem{cor}[defin]{Corollary}
\newtheorem{lem}[defin]{Lemma}
\newtheorem{thm}[defin]{Theorem}

